Linear Network Coding over Rings, Part I: Scalar Codes and Commutative Alphabets

Fixed-size commutative rings are quasi-ordered such that all scalar linearly solvable networks over any given ring are also scalar linearly solvable over any higher-ordered ring. As consequences, if a network has a scalar linear solution over some finite commutative ring, then (i) the network is also scalar linearly solvable over a maximal commutative ring of the same size, and (ii) the (unique) smallest size commutative ring over which the network has a scalar linear solution is a field. We prove that a commutative ring is maximal with respect to the quasi-order if and only if some network is scalar linearly solvable over the ring but not over any other commutative ring of the same size. Furthermore, we show that maximal commutative rings are direct products of certain fields specified by the integer partitions of the prime factor multiplicities of the maximal ring's size. Finally, we prove that there is a unique maximal commutative ring of size $m$ if and only if each prime factor of $m$ has multiplicity in $\{1,2,3,4,6\}$. In fact, whenever $p$ is prime and $k \in \{1,2,3,4,6\}$, the unique such maximal ring of size $p^k$ is the field $GF(p^k)$. However, for every field $GF(p^k)$ with $k\not\in \{1,2,3,4,6\}$, there is always some network that is not scalar linearly solvable over the field but is scalar linearly solvable over a commutative ring of the same size. These results imply that for scalar linear network coding over commutative rings, fields can always be used when the alphabet size is flexible, but alternative rings may be needed when the alphabet size is fixed.

==> tab_plot28.tex <==
% A table of the maximal partitions of k, for k <= 30
\begin{table}[h!]
\small
 \begin{center}
  \begin{tabular}{|l|}
  \hline
  (1) 
  \\ \hline
  (2) 
  \\ \hline
  (3) 
  \\ \hline
  (4) 
  \\ \hline
  (5) \
    (3,2) 
  \\ \hline
  (6) 
  \\ \hline
  (7) \ 
    (5,2) \
    (4,3) 
  \\ \hline
  (8) \
    (5,3) 
  \\ \hline
  (9) \ 
      (7,2) \
      (5,4) 
  \\ \hline
  (10) \
      (7,3) \
      (6,4) 
  \\ \hline
  (11) \
      (9,2) \
      (8,3) \ 
      (7,4) \
      (6,5) 
  \\ \hline
  (12) \
      (7,5) 
  \\ \hline
  (13) \ 
      (11,2) \ 
      (10,3) \
      (9,4) \
      (8,5) \ 
      (7,6) 
  \\ \hline
  (14) \
      (11,3) \
      (10,4) \ 
      (9,5) \
      (8,6) 
  \\ \hline
  (15) \
      (13,2) \
      (11,4) \
      (9,6) \
      (8,7) 
  \\ \hline
  (16) \
      (13,3) \
      (11,5) \
      (10,6) \
      (9,7) 
  \\ \hline
  (17) \
      (15,2) \
      (14,3) \
      (13,4) \
      (12,5) \
      (11,6) \
      (10,7) \
      (9,8) \
      (7,6,4) 
  \\ \hline
  (18) \
      (14,4) \
      (13,5) \
      (11,7) \
      (10,8) 
  \\ \hline
  (19) \
      (17,2) \
      (16,3) \
      (15,4) \
      (14,5) \
      (13,6) \
      (12,7) \
      (11,8) \
      (10,9) \
      (9,6,4) \
      (8,6,5) 
  \\ \hline
  (20) \
      (17,3) \
      (14,6) \
      (13,7) \
      (12,8) \
      (11,9) 
  \\ \hline
  (21) \
      (19,2) \
      (17,4) \
      (16,5) \
      (15,6) \
      (13,8) \
      (12,9) \
      (11,10) \
      (11,6,4) 
  \\ \hline
  (22) \
      (19,3) \
      (18,4) \
      (17,5) \
      (16,6) \
      (15,7) \
      (14,8) \
      (13,9) \
      (12,10) \
      (9,8,5) \
      (9,7,6) 
  \\ \hline
  (23) \
      (21,2) \
      (20,3) \
      (19,4) \
      (18,5) \
      (17,6) \
      (16,7) \
      (15,8) \
      (14,9) \
      (13,10) \ 
      (13,6,4) 
      \\ \hspace{7.5mm}
      (12,11) \
      (11,7,5) \ 
      (10,9,4) \ 
      (10,7,6) \
      (9,8,6) 
  \\ \hline
  (24) \
    (19,5) \
    (17,7) \
    (15,9) \
    (14,10) \
    (13,11) \ 
  \\ \hline
  (25) \ 
    (23,2) \ 
    (22,3) \
    (21,4) \
    (19,6) \
    (18,7) \
    (17,8) \
    (16,9) \ 
    (15,10) \ 
    (15,6,4) \ 
    (14,11) 
    \\ \hspace{7.5mm}
    (13,12) \
    (11,10,4) \ 
    (11,8,6) \
    (10,9,6) \
    (10,8,7) \
  \\ \hline
  (26) \
    (23,3) \ 
    (22,4) \
    (21,5) \
    (20,6) \
    (19,7) \
    (18,8) \
    (17,9) \
    (16,10) \ 
    (15,11) 
    \\ \hspace{7.5mm}
    (14,12) \
    (12,9,5) \ 
    (11,9,6) \
    (11,8,7) \
    (10,9,7) \
  \\ \hline
  (27) \
    (25,2) \
    (23,4) \
    (22,5) \
    (21,6) \
    (20,7) \
    (19,8) \
    (17,10) \
    (17,6,4) \ 
    (16,11) 
    \\ \hspace{7.5mm}
    (15,12) \
    (14,13) \
    (14,8,5) \ 
    (13,10,4) \ 
    (13,8,6) \
    (12,8,7) \
    (11,10,6) \ 
  \\ \hline
  (28) \
    (25,3) \ 
    (23,5) \
    (22,6) \
    (20,8) \
    (19,9) \
    (18,10) \ 
    (17,11) \
    (16,12) \
    (15,13) 
    \\ \hspace{7.5mm}
    (13,9,6) \ 
    (12,11,5) \ 
    (11,9,8) \
  \\ \hline
  (29) \
    (27,2) \
    (26,3) \
    (25,4) \
    (24,5) \
    (23,6) \
    (22,7) \
    (21,8) \
    (20,9) \
    (19,10) \
    (19,6,4) 
    \\ \hspace{7.5mm}
    (18,11) \
    (17,12) \
    (16,13) \
    (16,7,6) \ 
    (15,14) \
    (15,10,4) \ 
    (15,8,6) \
    (14,11,4) 
    \\ \hspace{7.5mm}
    (14,9,6) \
    (13,11,5) \
    (13,10,6) \ 
    (13,9,7) \
    (12,10,7) \ 
    (12,9,8) \
    (11,10,8) \
  \\ \hline
  (30) \
    (26,4) \
    (23,7) \
    (22,8) \
    (21,9) \
    (19,11) \
    (18,12) \
    (17,13) \
    (16,14) \
    (13,9,8) \
    (12,11,7) \
  \\ \hline
     \end{tabular}
 \end{center}
  \caption{The maximal partitions of $k = 1,2,\dots,30$ under partition division.}
  \label{tab:1}
\end{table}

\begin{figure}[h!]
\begin{tikzpicture}
  %
  \begin{semilogyaxis}
  [height=10.5cm,
  width=16cm,
  grid=major,
  xmin = 1, xmax= 100,
  ymin = 1, ymax = 1000000000,
  %axis y line*=left,
  ylabel={Number of (maximal) partitions of $k$},
  ylabel near ticks,
  legend pos = north west]
  %
  %\addlegendimage{/pgfplots/refstyle=Pplot}\addlegendentry{partitions}
  \addplot[color=black, mark = *, only marks]
  %
  coordinates {
    (1, 1)
    (2, 1)
    (3, 1)
    (4, 1)
    (5, 2)
    (6, 1)
    (7, 3)
    (8, 2)
    (9, 3)
    (10, 3)
    (11, 5)
    (12, 2)
    (13, 6)
    (14, 5)
    (15, 5)
    (16, 5)
    (17, 9)
    (18, 5)
    (19, 11)
    (20, 6)
    (21, 9)
    (22, 11)
    (23, 16)
    (24, 6)
    (25, 16)
    (26, 15)
    (27, 17)
    (28, 13)
    (29, 26)
    (30, 11)
    (31, 30)
    (32, 19)
    (33, 27)
    (34, 28)
    (35, 32)
    (36, 17)
    (37, 45)
    (38, 37)
    (39, 41)
    (40, 27)
    (41, 58)
    (42, 29)
    (43, 65)
    (44, 43)
    (45, 52)
    (46, 60)
    (47, 81)
    (48, 37)
    (49, 83)
    (50, 61)
    (51, 82)
    (52, 68)
    (53, 110)
    (54, 63)
    (55, 105)
    (56, 71)
    (57, 110)
    (58, 107)
    (59, 146)
    (60, 61)
    (61, 159)
    (62, 127)
    (63, 135)
    (64, 114)
    (65, 166)
    (66, 109)
    (67, 206)
    (68, 143)
    (69, 191)
    (70, 138)
    (71, 245)
    (72, 112)
    (73, 264)
    (74, 208)
    (75, 225)
    (76, 197)
    (77, 291)
    (78, 181)
    (79, 339)
    (80, 187)
    (81, 306)
    (82, 285)
    (83, 398)
    (84, 182)
    (85, 382)
    (86, 332)
    (87, 394)
    (88, 284)
    (89, 502)
    (90, 240)
    (91, 502)
    (92, 361)
    (93, 491)
    (94, 447)
    (95, 561)
    (96, 295)
    (97, 670)
    (98, 467)
    (99, 592)
    (100, 417)
  }; \addlegendentry{Maximal partitions}
  \addplot[color=red]
  coordinates {
      (1,1)
    (2,2)
    (3,3)
    (4,5)
    (5,7)
    (6,11)
    (7,15)
    (8,22)
    (9,30)
    (10, 42)
    (11, 56)
    (12, 77)
    (13, 101)
    (14, 135)
    (15, 176)
    (16, 231)
    (17, 297)
    (18, 385)
    (19, 490)
    (20, 627)
    (21, 792)
    (22, 1002)
    (23, 1255)
    (24, 1575)
    (25, 1958)
    (26, 2436)
    (27, 3010)
    (28, 3718)
    (29, 4565)
    (30, 5604)
    (31, 6842)
    (32, 8349)
    (33, 10143)
    (34, 12310)
    (35, 14883)
    (36, 17977)
    (37, 21637)
    (38, 26015)
    (39, 31185)
    (40, 37338)
    (41, 44583)
    (42, 53174)
    (43, 63261)
    (44, 75175)
    (45, 89134)
    (46, 105558)
    (47, 124754)
    (48, 147273)
    (49, 173525)
    (50, 204226)
    (51, 239943)
    (52, 281589)
    (53, 329931)
    (54, 386155)
    (55, 451276)
    (56, 526823)
    (57, 614154)
    (58, 715220)
    (59, 831820)
    (60, 966467)
    (61, 1121505)
    (62, 1300156)
    (63, 1505499)
    (64, 1741630)
    (65, 2012558)
    (66, 2323520)
    (67, 2679689)
    (68, 3087735)
    (69, 3554345)
    (70, 4087968)
    (71, 4697205)
    (72, 5392783)
    (73, 6185689)
    (74, 7089500)
    (75, 8118264)
    (76, 9289091)
    (77, 10619863)
    (78, 12132164)
    (79, 13848650)
    (80, 15796476)
    (81, 18004327)
    (82, 20506255)
    (83, 23338469)
    (84, 26543660)
    (85, 30167357)
    (86, 34262962)
    (87, 38887673)
    (88, 44108109)
    (89, 49995925)
    (90, 56634173)
    (91, 64112359)
    (92, 72533807)
    (93, 82010177)
    (94, 92669720)
    (95, 104651419)
    (96, 118114304)
    (97, 133230930)
    (98, 150198136)
    (99, 169229875)
    (100, 190569292)
    }; \addlegendentry{Partitions}
  \end{semilogyaxis}
\end{tikzpicture}
\caption{Plots of the number of partitions and the number of maximal partitions of $k$.}
\label{fig:anti_prime}
\end{figure}

